Spectral Evolution and Photo-ionization Analysis of Nova Cas 2020 (V1391 Cas)

We present spectroscopic observations of Nova Cas 2020(V1391 Cas) obtained using the Russian Turkish Telescope during different stages of its 2020 outburst. We followed the spectral evolution of the nova until it entered the nebular phase. The expansion velocity of the ejecta reached $\sim$780 $\mathrm{km\,s^{-1}}$. The fluxes of the neutral [O I] lines at wavelengths 6300, 6364, and 5577 $\r{A}$ were used to calculate the electron temperature and the mass of neutral oxygen in the ejecta. We found average values $T_e = 4890\,K$ ,$M_{OI} = 2.54 \times 10^{-5}\, M_{\odot}$ which are consistent with the values calculated for other novae. We modeled the nova's ejected envelope 515 days after its discovery and found that the log elemental abundances by number relative to Hydrogen of the envelope are He = -0.7, C = -5.5, O = -2.5, N = -2.0 and Ne = -4.0.

==> extra_biblio.tex <==

From Aydi 2020 paper (The slow component is the pre-maximum p Cygni )

From Aydi 2020 paper (premaximum P Cygni proﬁle the
“slow component” and the postmaximum broad emission higher-velocity P Cygni absorption the “fast component.”)

therfore the nova is expected to (((recovery in brightness to a fainter level than the start of t))) (((This dust will effectively block out
the light from the photosphere interior to it, causing the sudden
drop of light. The recovery to the previous decline is caused by
the geometric dilution of the dust as the shell expands, allowing
the photosphere to be seen again with little extinction.)))


A class that contains well studied dust forming novae like V705 Cas and  this is characterised by dust dips in the light curve consistent with our observations on........ novae of. 

period is equal to .... 3.803568h 0.158482d ()cite 


V476 Cyg ...
OS And  ...
V1370 Aql ...
V1419 Aql ...
V2274 Cyg ...
QV Vul  ...
V842 Cen 0.164
NQ Vul  ... 0.146501
LW Ser  ...
FH Ser  ...
V705 Cas 0.228
V732 Sgr ...
T Aur 0.204
DQ Her 0.194
V992 Sco 0.154
V445 Pup 0.65065


from nova 339del paper(The asymmetry of the line profiles at this stage, with the red
side brighter than the blue side, is caused by the still high optical
depth of the gas. At the same time, the appearance of forbid-
den lines from [N I] and [O I] marks the transition towards the
“nebular”, optically thin phase of the nova shell. The appearance
of the lines in this phase remains approximately constant. H α
(Fig. 6) no longer exhibits a true P-Cyg profile, but rather a heav-
ily dimmed blue side.)


(The emission profiles in the late phase show a clear signature of the non-sphericity of the ejecta, with several
lines also showing asymmetry between the red and blue sides.
The diﬀerent ionization species empirically describe ejecta ma-
terial of diﬀerent excitation energy, to complete our insight into
a very complex dynamical and geometrical structure of the ex-
panding nova envelope.)

optically thin phase

transition phase 


optically thin phase


we adopt a value of the ratio of 2.83216374 leading to a value ot tau = 0.17616097351874682 then the temperature 5271.84245018, 4635.34027343, 4772.54465439
leading to a mass of

array([1.65626302e-05, 6.00550166e-05, 2.54518274e-06])




\begin{table}
\caption[]{Cloudy Initial Values.}    
\label{tab:absorption}
%\begin{center}
\begin{tabular}{lc}
\hline \hline
Hydrogen Density    &  \\
Effective Temperature &        \\
Luminosity  &         \\
Filling Factor &       \\
Inner Radius &       \\
Helium Abundance &        \\
Carbon Abundance &      \\
Oxygen Abundance &      \\
Nitrogen Abundance &      \\
Neon Abundance  &       \\
\hline 
\end{tabular}
%\end{center}
\end{table} 



%\begin{thebibliography}{}


\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\providecommand{\url}[1]{\href{#1}{#1}}
\providecommand{\dodoi}[1]{doi:~\href{http://doi.org/#1}{\nolinkurl{#1}}}
\providecommand{\doeprint}[1]{\href{http://ascl.net/#1}{\nolinkurl{http://ascl.net/#1}}}
\providecommand{\doarXiv}[1]{\href{https://arxiv.org/abs/#1}{\nolinkurl{https://arxiv.org/abs/#1}}}

\bibitem[{{Astropy Collaboration} {et~al.}(2013){Astropy Collaboration},
  {Robitaille}, {Tollerud}, {Greenfield}, {Droettboom}, {Bray}, {Aldcroft},
  {Davis}, {Ginsburg}, {Price-Whelan}, {Kerzendorf}, {Conley}, {Crighton},
  {Barbary}, {Muna}, {Ferguson}, {Grollier}, {Parikh}, {Nair}, {Unther},
  {Deil}, {Woillez}, {Conseil}, {Kramer}, {Turner}, {Singer}, {Fox}, {Weaver},
  {Zabalza}, {Edwards}, {Azalee Bostroem}, {Burke}, {Casey}, {Crawford},
  {Dencheva}, {Ely}, {Jenness}, {Labrie}, {Lim}, {Pierfederici}, {Pontzen},
  {Ptak}, {Refsdal}, {Servillat}, \& {Streicher}}]{astropy:2013}
{Astropy Collaboration}, {Robitaille}, T.~P., {Tollerud}, E.~J., {et~al.} 2013,
  \aap, 558, A33, \dodoi{10.1051/0004-6361/201322068}

\bibitem[{{Astropy Collaboration} {et~al.}(2018){Astropy Collaboration},
  {Price-Whelan}, {Sip{H{o}}cz}, {G{"u}nther}, {Lim}, {Crawford}, {Conseil},
  {Shupe}, {Craig}, {Dencheva}, {Ginsburg}, {Vand erPlas}, {Bradley},
  {P{'e}rez-Su{'a}rez}, {de Val-Borro}, {Aldcroft}, {Cruz}, {Robitaille},
  {Tollerud}, {Ardelean}, {Babej}, {Bach}, {Bachetti}, {Bakanov}, {Bamford},
  {Barentsen}, {Barmby}, {Baumbach}, {Berry}, {Biscani}, {Boquien}, {Bostroem},
  {Bouma}, {Brammer}, {Bray}, {Breytenbach}, {Buddelmeijer}, {Burke},
  {Calderone}, {Cano Rodr{'i}guez}, {Cara}, {Cardoso}, {Cheedella}, {Copin},
  {Corrales}, {Crichton}, {D'Avella}, {Deil}, {Depagne}, {Dietrich}, {Donath},
  {Droettboom}, {Earl}, {Erben}, {Fabbro}, {Ferreira}, {Finethy}, {Fox},
  {Garrison}, {Gibbons}, {Goldstein}, {Gommers}, {Greco}, {Greenfield},
  {Groener}, {Grollier}, {Hagen}, {Hirst}, {Homeier}, {Horton}, {Hosseinzadeh},
  {Hu}, {Hunkeler}, {Ivezi{'c}}, {Jain}, {Jenness}, {Kanarek}, {Kendrew},
  {Kern}, {Kerzendorf}, {Khvalko}, {King}, {Kirkby}, {Kulkarni}, {Kumar},
  {Lee}, {Lenz}, {Littlefair}, {Ma}, {Macleod}, {Mastropietro}, {McCully},
  {Montagnac}, {Morris}, {Mueller}, {Mumford}, {Muna}, {Murphy}, {Nelson},
  {Nguyen}, {Ninan}, {N{"o}the}, {Ogaz}, {Oh}, {Parejko}, {Parley}, {Pascual},
  {Patil}, {Patil}, {Plunkett}, {Prochaska}, {Rastogi}, {Reddy Janga},
  {Sabater}, {Sakurikar}, {Seifert}, {Sherbert}, {Sherwood-Taylor}, {Shih},
  {Sick}, {Silbiger}, {Singanamalla}, {Singer}, {Sladen}, {Sooley},
  {Sornarajah}, {Streicher}, {Teuben}, {Thomas}, {Tremblay}, {Turner},
  {Terr{'o}n}, {van Kerkwijk}, {de la Vega}, {Watkins}, {Weaver}, {Whitmore},
  {Woillez}, {Zabalza}, \& {Astropy Contributors}}]{astropy:2018}
{Astropy Collaboration}, {Price-Whelan}, A.~M., {Sip{H{o}}cz}, B.~M., {et~al.}
  2018, aj, 156, 123, \dodoi{10.3847/1538-3881/aabc4f}

\bibitem[{{Aydi} {et~al.}(2020){Aydi}, {Chomiuk}, {Izzo}, {Harvey},
  {Leahy-McGregor}, {Strader}, {Buckley}, {Sokolovsky}, {Kawash}, {Kochanek},
  {Linford}, {Metzger}, {Mukai}, {Orio}, {Shappee}, {Shishkovsky}, {Steinberg},
  {Swihart}, {Sokoloski}, {Walter}, \& {Woudt}}]{2020ApJ...905...62A}
{Aydi}, E., {Chomiuk}, L., {Izzo}, L., {et~al.} 2020, \apj, 905, 62,
  \dodoi{10.3847/1538-4357/abc3bb}
  
\bibitem[{{Banerjee} {et al.}(2020){Banerjee}}]{{2020ATel14006....1B}} {Banerjee}, D. P. K., Shahbandeh, M., Evans, A., Hsiao, E. 2020, ATel, 14006, 1

\bibitem[{{Banerjee} {et~al.}(2020){Banerjee}, {Anupama}, {Munari}, {Ghosh},
  {Omar}, \& {DOT Team}}]{2020ATel14272....1B}
{Banerjee}, D.~P.~K., {Anupama}, G.~C., {Munari}, U., {et~al.} 2020, The
  Astronomer's Telegram, 14272, 1

\bibitem[{Bradley {et~al.}(2020)Bradley, Sip{\H o}cz, Robitaille, Tollerud,
  Vin{\'{\i}}cius, Deil, Barbary, Wilson, Busko, G{\"u}nther, Cara, Conseil,
  Bostroem, Droettboom, Bray, Bratholm, Lim, Barentsen, Craig, Pascual, Perren,
  Greco, Donath, de~Val-Borro, Kerzendorf, Bach, Weaver, D'Eugenio, Souchereau,
  \& Ferreira}]{larry_bradley_2020_4044744}
Bradley, L., Sip{\H o}cz, B., Robitaille, T., {et~al.} 2020, astropy/photutils:
  1.0.0, 1.0.0,  Zenodo, \dodoi{10.5281/zenodo.4044744}

\bibitem[{{Cayrel}(1988)}]{1988IAUS..132..345C}
{Cayrel}, R. 1988, in The Impact of Very High S/N Spectroscopy on Stellar
  Physics, ed. G.~{Cayrel de Strobel} \& M.~{Spite}, Vol. 132, 345

\bibitem[{Craig {et~al.}(2017)Craig, Crawford, Seifert, Robitaille, Sip{\H
  o}cz, Walawender, Vin{\'{\i}}cius, Ninan, Droettboom, Youn, Tollerud, Bray,
  Walker, Janga, Stotts, G{\"u}nther, Rol, Bach, Bradley, Deil, Price-Whelan,
  Barbary, Horton, Schoenell, Heidt, Gasdia, Nelson, \&
  Streicher}]{matt_craig_2017_1069648}
Craig, M., Crawford, S., Seifert, M., {et~al.} 2017, astropy/ccdproc:
  v1.3.0.post1, \dodoi{10.5281/zenodo.1069648}

\bibitem[{{Della Valle & Livio}(1995){Della Valle & Livio}}]{1995ApJ...452..704D}
{Della Valle}, M., {Livio}, M. 1995, The Calibration of Novae as Distance Indicators, \apj 452, 704-709, \dodoi{10.1086/176342}

\bibitem[{{Della Valle & Livio}(1998){Della Valle & Livio}}]{1998ApJ...506..818D}
{Della Valle}, M., {Livio}, M. 1998, The Spectroscopic Differences between Disk and Thick-Disk/Bulge Novae, \apj 506, 818-823, \dodoi{10.1086/306275}

\citet{2021OEJV..220...37D}
\bibitem[{{Dubovsky} {et~al.}(2021){Dubovsky}, {Medulka}, \& {Kudzej}}]{2021OEJV..220...37D}
{Dubovsky}, P.~A., {Medulka}, T., \& {Kudzej}, I. 2021, Vol.~220, Open European Journal on Varıable Stars, Proceedings of the 52nd Conference on Variable Stars Research, ed. R. {Kocian}, 37,
  \dodoi{10.5817/OEJV2021-0220}

\bibitem[{{Esenoglu}(1997){Esenoglu}}]{1996PASP..109.1285E} {Esenoglu}, H. H. 1997, Dissertation summary \PASP, 109, 1285, \dodoi{10.1086/134009}

\bibitem[{{Evans} {et~al.}(2005){Evans}, {Tyne}, {Smith}, {Geballe}, {Rawlings}, \& {Eyres}}]{2005MNRAS.360.1483E} {Evans}, A., {Tyne}, V.~H., {Smith}, O., {et~al.} 2005, \mnras, 360, 1483, \dodoi{10.1111/j.1365-2966.2005.09146.x}

\bibitem[{{Fitzpatrick} {et~al.}(2019){Fitzpatrick}, {Massa}, {Gordon},
  {Bohlin}, \& {Clayton}}]{2019ApJ...886..108F}
{Fitzpatrick}, E.~L., {Massa}, D., {Gordon}, K.~D., {Bohlin}, R., \& {Clayton},
  G.~C. 2019, \apj, 886, 108, \dodoi{10.3847/1538-4357/ab4c3a}

\bibitem[{{Fujii} {et~al.}(2020){Fujii}}]{2020ATel13941....1F} {Fujii}, M., Arai, A., Kawakita, H. 2020, ATel, 13941, 1

\bibitem[{{Fujii} {et~al.}(2021){Fujii}}]{2021ApJ...907...70F} {Fujii}, M., {Arai}, A., {Kawakita}, H. 2021, \apj, 907, 70,
  \dodoi{10.3847/1538-4357/abd02e}

\bibitem[{{Jack} {et~al.}(2020){Jack}, {Schr{\"o}der}, {Eenens}, {Wolter},
  {Gonz{\'a}lez-P{\'e}rez}, {Schmitt}, \& {Hauschildt}}]{2020AN....341..781J}
{Jack}, D., {Schr{\"o}der}, K.-P., {Eenens}, P., {et~al.} 2020, Astronomische
  Nachrichten, 341, 781, \dodoi{10.1002/asna.202013818}

\bibitem[{{Hamed} {et al.}(2020){Hamed}}]{2020ATel13998....1H} {Hamed}, G. M., Esenoglu, H. H., Galeev, A. I. 2020, ATel, 13998, 1

\bibitem[{{Kawakita & Arai}(2017){Kawakita & Arai}}]{2017PoS...64.....1K}
{Kawakita}, H., {Arai}, A. 2017, in The Golden Age of Cataclysmic Variables and Related Objects IV

\bibitem[{{Khamitov} {et~al.}(2020){Khamitov}, {Bikmaev}, {Burenin},
  {Glushkov}, {Melnikov}, \& {Lyapin}}]{2020AstL...46....1K}
{Khamitov}, I.~M., {Bikmaev}, I.~F., {Burenin}, R.~A., {et~al.} 2020, Astronomy
  Letters, 46, 1, \dodoi{10.1134/S106377372001003X}

\bibitem[{{Kolb}(2020){Kolb}}]{2020BAV4/2020..193K} {Kolb}, M. 2020, BAV Rundbrief, 4/2020, 193-199

\bibitem[{Kramida {et~al.}(2020)Kramida, {Yu.~Ralchenko}, Reader, \& {and NIST
  ASD Team}}]{NIST_ASD}
Kramida, A., {Yu.~Ralchenko}, Reader, J., \& {and NIST ASD Team}. 2020, {NIST
  Atomic Spectra Database (ver. 5.8), [Online]. Available:
  {\tt{https://physics.nist.gov/asd}} [2020, November 3]. National Institute of
  Standards and Technology, Gaithersburg, MD.}

\bibitem[{{Lenz} \& {Ayres}(1992)}]{1992PASP..104.1104L}
{Lenz}, D.~D., \& {Ayres}, T.~R. 1992, \pasp, 104, 1104, \dodoi{10.1086/133096}

\bibitem[{McCully {et~al.}(2018)McCully, Crawford, Kovacs, Tollerud, Betts,
  Bradley, Craig, Turner, Streicher, Sipocz, Robitaille, \&
  Deil}]{curtis_mccully_2018_1482019}
McCully, C., Crawford, S., Kovacs, G., {et~al.} 2018, astropy/astroscrappy:
  v1.0.5 Zenodo Release, v1.0.5,  Zenodo, \dodoi{10.5281/zenodo.1482019}

\bibitem[{{McLaughlin}(1965){McLaughlin}}]{1965POMic...9..113M}
{McLaughlin}, B. 1965, \POMic, 9, 113

\bibitem[{{Munari} {et~al.}(2010){Munari}, {Henden}, {Valisa}, {Dallaporta}, \&
  {Righetti}}]{2010PASP..122..898M}
{Munari}, U., {Henden}, A., {Valisa}, P., {Dallaporta}, S., \& {Righetti},
  G.~L. 2010, \pasp, 122, 898, \dodoi{10.1086/655667}

\bibitem[{{Munari} {et~al.}(2020){Munari}, {Siviero}, {Vagnozzi}, {Sokolovsky},
  \& {Aydi}}]{2020ATel13905....1M}
{Munari}, U., {Siviero}, A., {Vagnozzi}, A., {Sokolovsky}, K., \& {Aydi}, E.
  2020, The Astronomer's Telegram, 13905, 1

\bibitem[{{Munari} {et al.}(2020){Munari}}]{{2020ATel14267....1M}} {Munari}, U., Banerjee, D. P. K., Castellani, F., Dallaporta, S., Maitan, A., Vagnozzi, A. 2020, ATel, 14267, 1

\bibitem[{{Oke}(1990)}]{1990AJ.....99.1621O}
{Oke}, J.~B. 1990, \aj, 99, 1621, \dodoi{10.1086/115444}

\bibitem[{{Russell} {et al.}(2020){Russell}}]{2020ATel13967....1R} {Russell}, W., Sitko, M. L., Rudy, R. J., Fujii, M., Arai, A., Kawakita, H. 2020, ATel, 13967, 1

\bibitem[{{Evans et al.}(2005){Evans et al.}}]{2005MNRAS.360.1483E} {Evans et al.}, A. and {Tyne}, V.~H. and {Smith}, O. and {Geballe}, T.~R. and {Rawlings}, J.~M.~C. and {Eyres}, S.~P.~S. 2005, Infrared spectroscopy of Nova Cassiopeiae 1993 - IV. A closer look at the dust, \mnras, 360, 1483, \dodoi{10.1111/j.1365-2966.2005.09146.x}

\bibitem[{{Schaefer}(2022){Schaefer}}]{2022MNRAS.517.6150S} {Schaefer}, B. E. 2022, Comprehensive catalogue of the overall best distances and properties of 402 galactic novae, \mnras, 517, 6150, \dodoi{110.1093/mnras/stac2900}

\bibitem[{{Selvelli} \& {Gilmozzi}(2019)}]{2019A&A...622A.186S}
{Selvelli}, P., \& {Gilmozzi}, R. 2019, \aap, 622, A186,
  \dodoi{10.1051/0004-6361/201834238}

\bibitem[{{Shore} {et al.}(1996){Shore}}]{2020ATel13939....1S} {Shore}, S. N., Boussin, C., Boyd, D., Buil, C., Lester, T., Michelet, J., Somogyi, P. (ARAS Group) 2020, ATel, 13939, 1

\bibitem[{Sokolovsky} {et~al.}(2020){Sokolovsky}, {Aydi}, {Izzo}, {Harvey}, {Atapin}, {Belinski}, {Dodin}, {Postnov}, {Potanin}, {Shatsky}, {Tatarnikov}, {Freour},
\{Wedderkopp}, {Kroer}, {Jundiyeh}, {Henriksen}, {Rasmussen}, {Quist}, {Madsen}, {Jepsen}, {Hartwigsen}, {Sorensen}, {Stovelbaek}, {Hansen}, {Otap}, {Iv}, {Kolborg}, %\{Fynbo}, {Keniger}, {Chomiuk}, {Kawash}, {Strader}, {Mukai}, {Li}, {Kafka}, {Karpov}, {Korotkiy}}]{2020ATel14004....1S}
{Sokolovsky}, K.V., {Aydi}, E., {Izzo}, E. {et~al.} 2020, The Astronomer's Telegram, 14004, 1

\bibitem[{{Sokolovsky} {et~al.}(2020){Sokolovsky}, {Chomiuk}, {Kawash}, {Aydi}, {Strader}, {Mukai}, {Li}, {Kafka}, {Karpov}, {Korotkiy}, {Stanek}, {Kochanek},
\& {Shappee}}]{2020ATel13919....1S}
{Sokolovsky}, K., {Chomiuk}, L., {Kawash}, A. {et~al.} 2020, The Astronomer's Telegram, 13919, 1

\bibitem[{{Sokolovsky} {et~al.}(2020){Sokolovsky}, {Aydi}, {Chomiuk}, {Kawash},
  {Strader}, {Atapin}, {Belinski}, {Dodin}, {Postnov}, {Potanin}, {Shatsky},
  {Munari}, \& {Korotkiy}}]{2020ATel13903....1S}
{Sokolovsky}, K., {Aydi}, E., {Chomiuk}, L., {et~al.} 2020, The Astronomer's
  Telegram, 13903, 1

\bibitem[{{Starrfield} {et~al.}(2016){Starrfield}, {Iliadis}, \&
  {Hix}}]{2016PASP..128e1001S}
{Starrfield}, S., {Iliadis}, C., \& {Hix}, W.~R. 2016, \pasp, 128, 051001,
  \dodoi{10.1088/1538-3873/128/963/051001}

\bibitem[{{Tanaka} {et~al.}(2011){Tanaka}, {Iliadis}}]{2011PASJ..63...911T}
{Tanaka}, J., {Nogami}, D., {Fujii}, M., {Ayani}, K., {Kato}, T., {Maehara}, H., {Kiyota}, S., {Nakajima}, K. 2011, \pasj, 63, 911,
  \dodoi{10.1093/pasj/63.4.911}

\bibitem[{{Tody}(1993)}]{1993ASPC...52..173T}
{Tody}, D. 1993, in Astronomical Society of the Pacific Conference Series,
  Vol.~52, Astronomical Data Analysis Software and Systems II, ed. R.~J.
  {Hanisch}, R.~J.~V. {Brissenden}, \& J.~{Barnes}, 173

\bibitem[{{van Dokkum}(2001)}]{2001PASP..113.1420V}
{van Dokkum}, P.~G. 2001, \pasp, 113, 1420, \dodoi{10.1086/323894}

\bibitem[{{Waagen}(2020){Waagen}}]{2020AAVSO715.....1W} {Waagen}, E. O. 2020, AAVSO Alert Notice, 715, 1

\bibitem[{{Warner}(2003)}]{2003cvs..book.....W}
{Warner}, B. 2003, Cataclysmic Variable Stars (Cambridge: Cambridge University
  Press), \dodoi{10.1017/CB09780511586491}

\bibitem[{{Wenzel}(2021){Wenzel}}]{{2021BAV.....1....1W}} {Wenzel}, K. 2021, BAV Rundbrief, 44-45

\bibitem[{{Williams}(1994)}]{1994ApJ...426..279W}
{Williams}, R.~E. 1994, \apj, 426, 279, \dodoi{10.1086/174062}

\bibitem[{{Woodward} {et al.}(2020){Woodward}}]{{2020ATel14034....1W}} {Woodward}, C. E., Banerjee, D. P. K., Evans, A. 2020, ATel, 14034, 1

\end{thebibliography}




%\bibliography{references.bib}
%\end{document}


